Scale setting for large-$N$ SUSY Yang-Mills on the lattice

In this paper we study the large $N$ limit of four-dimensional Supersymmetric Yang-Mills on the lattice using twisted reduced models. We have generated configurations with dynamical massive gluinos and various lattice 't Hooft couplings, and verified that the Pfaffian remains positive. We have determined the lattice spacing in terms of various observables obtaining compatible results. Extrapolating to the massless gluino limit we obtain the lattice spacing dependence on the bare couplings for the supersymmetric theory. The observed dependence goes along the expected behaviour predicted by perturbation theory.

==> body/8-aux.tex <==

By performing the integration, one is left with the following dependence of the scale on the 't Hooft coupling at leading order in perturbation theory:
\begin{equation}\label{eqn:logapt}
    % -\log{a} = \frac{24\pi^2}{b_0\lambda} + \frac{\lambda}{3} + \log\Lambda
    - \log{a} = \frac{1}{b_0\lambda} + \frac{b_1}{b_0^2}\log{\lambda} + \frac{b_1\log{(b_1\lambda+b_0)}}{b_0^2} + \log\Lambda
\end{equation}
\textcolor{red}{check this formula}
%  Since $b_0$ has a definite numerical value, one can perform a 1 parameter fit, extracting only the overall shift $\log\Lambda$. Alternatively one can perform a 2 parameters fit and extracting also $b_0$ and then confront its fitted value with the expected one. 
Another possibility is to use the analytical form of the Novikov-Shifman-Vainshtein-Zakharov (NSVZ) $\beta$-function \cite{Novikov:1983uc}, coming from instanton calculation
 \begin{equation}
     \beta(\lambda) = -\frac{3}{16\pi^2}\frac{\lambda^2}{1-\frac{\lambda}{8\pi^2}}
 \end{equation}
 which leads to  \textcolor{red}{check the overall factor 2}
 \begin{equation}\label{eqn:logaNSVZ}
    -\log{a} = \frac{1}{3}\qty(\frac{8\pi^2}{\lambda}+\log{\lambda}) + \log\Lambda
 \end{equation}
in which there are no free coefficients, apart from the overall shift. There is another improvement that can be made. The 't Hooft coupling is defined as $\sfrac{1}{b}$ and the fit with \eqref{eqn:logapt} or \eqref{eqn:logaNSVZ} could be performed with this definition. However, it is well-known that, on the lattice, perturbative scaling works better using an improved lattice coupling constant $\lambda_I=\sfrac{1}{b_I(b)}$, whose definition is not unique. Many options have been put forward and tested in the literature, the one we used is \cite{Allton:2007py}
% \begin{align}
%     \lambda_I^{(1)} &= \frac{1}{b P(b)} \label{eqn:allton}\\ 
%     \lambda_I^{(2)} &= 8(1-P(b)) \label{eqn:parisi}
% \end{align}
\begin{equation}
    \lambda_I = \frac{1}{b P(b)} \label{eqn:allton}
\end{equation}
where $P(b)$ represent the average value of the plaquette extrapolated in the massless-gluino limit. %We performed our analysis with both the definition of the improved coupling, obtaining compatible results. We are going to present the result for $\lambda_I^{(1)}$. 
\textcolor{red}{Other definition for the improved coupling?}

In Fig.~\ref{} \textcolor{red}{add plot} we display the dependence of the logarithm of the lattice spacing on the improved coupling $\lambda_I^{(1)}$. We performed an initial 2 parameter fit with the functional form in Eq.~\eqref{eqn:logapt} setting $b_1=0$, from which we extracted $3(4\pi)^2b_0 = 10.46(85)$ with a reduced $\chi^2=1.17$. We remind that the theoretical expectation for the coefficient is $3(4\pi)^2b_0 = 11 - 4N_f$, where $N_f$ is the number of Dirac adjoint flavors. Our number sits in between 11, i.e. the pure Yang-Mills theory ($N_f=0$), and 9, i.e. a theory with one Majorana $N_f=\sfrac{1}{2}$. \textcolor{red}{fit at 2 loops}. On the other hand, we also perform a fit with Eq.~\ref{eqn:logaNSVZ}, extracting only the overall parameter. We obtained a reduced $\chi^2=1.2$.

\textcolor{red}{Write some overall conclusion}

